Finfluencers on TikTok: A Longitudinal Analysis of Content, Engagement, and Disclaimer Practices

The rise of social media financial influencers (finfluencers) has transformed how financial information is disseminated to broad and often inexperienced audiences. While these creators may contribute to financial literacy, concerns remain regarding the reliability of their content and the adequacy of risk disclosures. Using data collected through TikTok's Research API, we analyze UK finfluencer content, engagement dynamics, disclaimer practices, audience sentiment, and network structure. The primary dataset comprises 13,215 videos and 104,097 comments posted by 71 UK-based finfluencers between April and September 2024, while a follow-up dataset covering October 2025 to March 2026 enables longitudinal analysis of disclaimer practices, engagement trends, and hashtag usage. Using topic modeling, we identify four dominant themes: Entrepreneurship \& Side Hustles, Property Investing, Active Trading, and Saving \& Budgeting. Sentiment analysis of audience comments reveals predominantly neutral-to-positive responses, while engagement analysis shows only a negligible association between video duration and engagement rate. Social network analysis indicates a collaborative ecosystem in which mid-tier finfluencers frequently act as bridges between creator groups. Explicit disclaimers and risk-related language remain relatively uncommon overall and are concentrated primarily in trading-related content. The findings highlight challenges related to financial transparency and disclosure practices within short-form financial content ecosystems. We discuss implications for consumer protection and the design of clearer and more standardized financial risk disclosures on social media platforms.

==> Introduction.tex <==
The rise of social media has transformed the dissemination of financial information, with so-called financial influencers (or for short finfluencers) playing an increasingly significant role in shaping public investment behaviour. Platforms such as TikTok and Instagram have become key sources of financial content, where influencers promote investment strategies, trading platforms, and cryptocurrency ventures to wide audiences, often without proper regulatory oversight \cite{2023insta,2024tiktokinsta}. While these influencers have the potential to democratise access to financial knowledge, concerns over misinformation, misleading promotions, and the risk of financial harm have drawn growing scrutiny from regulators.

In response to these challenges, the UK's Financial Conduct Authority (FCA) has strengthened its oversight of financial promotions on social media, emphasising that all investment-related content must be fair, clear, and not misleading. Recent enforcement actions, including interviews under caution and legal proceedings against finfluencers, signal a move towards stricter regulation \cite{FCA2024}. This paper examines the intersection of financial advice, influencer marketing, and regulatory policy, assessing the effectiveness of existing measures in protecting consumers while promoting responsible financial communication in digital spaces.

TikTok remains the most popular social media platform globally, evidenced by its leading position in mobile application downloads. In 2024, it recorded 773 million downloads, surpassing all other social apps and reinforcing its dominance in the digital ecosystem \cite{businessofapps2024}.

Previous research has examined influencer marketing effectiveness on TikTok, often focusing on entertainment-oriented traits such as humour and originality (e.g., \cite{BARTA2023}), as well as the platform’s structural impact on creative labour and content commodification \cite{Hayes2024}. This study shifts the focus to finfluencers in the UK, analyzing their content strategies, follower interactions, and implications for financial literacy and consumer protection. It identifies behavioural patterns, risks, and communication strategies, offering empirically grounded recommendations for safer, more transparent financial communication. Given TikTok’s popularity among teenagers and young adults \cite{2020Tiktokpopular}, understanding the influence of finfluencers—who often provide financial advice that may inadvertently cause harm or regulatory non-compliance—is crucial for safeguarding financial well-being and ensuring appropriate oversight of financial content on social media.

\subsection{Our contribution}
Our contribution can be summarised as follows:

\begin{itemize} \item A TikTok dataset consisting of: \begin{itemize} \item Data on 71 finfluencer accounts identified as providing some form of financial advice in the UK during the six-month period between April and September 2024. 
\item Metadata and extracted textual content (e.g., descriptions, voice\_to\_text transcripts) for 13,216 videos posted by these 71 users during the same period.
\item Video comment data for these 13,216 videos, totalling 104,097 comments. 
\end{itemize} 
\item Our data analysis includes: 
\begin{itemize} \item Analysis of video engagements and topics. 

\item A social graph of the finfluencers, i.e., who among them follows whom. \item Analysis of the existence of disclaimers in the video and bio content of these users. 
\item Sentiment analysis of the video comments. 
\end{itemize} 

\end{itemize}

\subsection*{Acknowledgment}  
The authors gratefully acknowledge funding from the {National Research Centre on Privacy, Harm Reduction and Adversarial Influence Online (REPHRAIN)}.
